Unsupervised Denoising for Signal-Dependent and Row-Correlated Imaging Noise

Accurate analysis of microscopy images is hindered by the presence of noise. This noise is usually signal-dependent and often additionally correlated along rows or columns of pixels. Current self- and unsupervised denoisers can address signal-dependent noise, but none can reliably remove noise that is also row- or column-correlated. Here, we present the first fully unsupervised deep learning-based denoiser capable of handling imaging noise that is row-correlated as well as signal-dependent. Our approach uses a Variational Autoencoder (VAE) with a specially designed autoregressive decoder. This decoder is capable of modeling row-correlated and signal-dependent noise but is incapable of independently modeling underlying clean signal. The VAE therefore produces latent variables containing only clean signal information, and these are mapped back into image space using a proposed second decoder network. Our method does not require a pre-trained noise model and can be trained from scratch using unpaired noisy data. We benchmark our approach on microscopy datatsets from a range of imaging modalities and sensor types, each with row- or column-correlated, signal-dependent noise, and show that it outperforms existing self- and unsupervised denoisers.

==> changes.tex <==
Reorganise results table. HDN in brackets
Diffusion prior for inverse probelms section in related work. How they are different, weaknesses. with forward model
GAN unpaired methods in related work.
Cite Noise2Self/self2self/neighbour2neighbour/SUPPRT w/ N2V.
Make related work inline. Refer to section 3.1 row correlated noise
Make experiements inline. 5.1 Comparing denoising. 5.2/3 Ablations
Fix arrow in fig 3
Make fig 3b clearer
Fix line in figure 5
Change scientific imageing to microscopy

==> sections/background-old.tex <==
\section{Background}
\label{sec:background}
\subsection{Image formation and imaging noise}
\label{sec:noise}
We can express image formation as a two step process.
The clean image, or as we also refer to it, the \emph{signal}, $\s=(s_{1,1}, \dots, s_{N,M})$, is drawn from a distribution $p(\s)$ and then subjected to noise, producing the noisy image $\x=(x_{1,1}, \dots, x_{N,M})$ as drawn from the noise distribution $p(\x|\s)$.
Here, $s_{i,j}$ and $x_{i,j}$ correspond to the respective pixel values at position $(i,j)$, and $N$ and $M$ are the number of rows and columns in the image, respectively.

Generally, we assume that the imaging noise is zero-centered, that is, the expected value of a noisy image equals the signal, $\mathbb{E}_{p(\x|\s)}[\x] = \s$. 
Note that zero-centered noise is a weak assumption that is widely shared in literature~(\eg~\cite{krull2019noise2void, laine2019high,eom2023statistically}).
Another way of looking at this assumption is that the sensor or camera is assumed to behave linearly so that an increase in $s_{i,j}$ (\eg by increasing the light intensity) will, on average, result in a proportional increase in $x_{i,j}$.

\noindent
{\bf Additive white Gaussian noise:}
Arguably, the most basic traditionally used noise model is additive white Gaussian (AWG) noise, see~\eg \cite{dabov2006image,buades2005non,metzler2018unsupervised}.
We can write the probability distribution for noisy observations in an AWG noise model as
\begin{equation}
    p(\x|\s) 
    = \prod_{i=1}^{N} \prod_{j=1}^{M} p(x_{i,j}|s_{i,j}),
    \label{eq:pixel-indep}
\end{equation}
formulated as a product over pixels.
In general, we refer to any type of noise model that can be factorised according to \cref{eq:pixel-indep} as spatially uncorrelated.
In AWG noise, $p(x_{i,j}|s_{i,j})$ corresponds to a normal distribution centered at $s_{i,j}$, with variance fixed for all $s_{i,j}$.

As a consequence, the AWG noise itself, $\n = \x-\s$, follows a fixed variance normal distribution centered at zero and is independent of the underlying signal. 
In general, we call noise that does not depend on the underlying signal, such that $p(\n|\s) = p(\n)$, signal-independent.
Types of noise for which this is not the case will be referred to as signal-dependent.

Denoising approaches have assumed noise to be both spatially uncorrelated and signal-independent.
Unfortunately, real imaging noise rarely follows these assumptions.

\noindent
{\bf Poisson shot noise:}
Most imaging systems are at least to some degree affected by Poisson shot noise~\cite{laine2021imaging}.
A Poisson noise model follows \cref{eq:pixel-indep}, with $p(x_{i,j}|s_{i,j})$ corresponding to a Poisson distribution with rate $\lambda=s_{i,j}$.
A popular variant on this model is the Poisson-Gaussian noise model (\eg~\cite{zhang2019poisson}), where $p(x_{i,j}|s_{i,j})$ is assumed to be a combination of Poisson shot noise and Gaussian read-out noise.

Poisson and Poisson-Gaussian noise models are spatially uncorrelated but signal-dependent, since the variance of the Poisson component in each pixel depends on the pixel's signal $s_{i,j}$.

\noindent
{\bf Row-correlated noise:}
While Poisson-Gaussian noise models are a popular choice in describing noise distributions, many imaging systems  (\eg EMCCD, sCMOS, or scanning microscopes) can produce noise that does not conform to \cref{eq:pixel-indep}, but is instead correlated along rows (or columns) of pixels.

We propose to describe such noise as
\begin{equation}
    p(\x|\s) 
    = \prod_{i=1}^{N} \prod_{j=1}^{M} 
    p(x_{i,j}|\s, x_{i,1},\dots,x_{i,j-1}),
    \label{eq:structured}
\end{equation}
where 
$p(x_{i,j}|\s, x_{i,1},\dots,x_{i,j-1})$
is the distribution of possible noisy pixel values $x_{i,j}$ conditioned on the signal, as well as all ``previous'' values in the same row, $i$.
While this model can describe interactions between pixels within the same row, pixels in different rows are (conditionally) independent (given a signal $\s$).
Note that in this formulation a pixel $x_{i,j}$ can depend on not only the signal in pixel $(i,j)$, as with shot noise, but on the entire image for more complex interactions.

In our work, we consider this type of noise as described in~\cref{eq:structured}, which we believe is a good model for many real scientific imaging data.

\subsection{Latent variable models and Variational Autoencoders}
\label{sec:vae}
A latent variable model, with parameters $\theta$, defines a probability distribution, $p_\theta(\x) \propto \pxz\pz$, over observed variables $\x$ via latent variables $\z$. 
This can be used to represent a data generation process in which a value $\z$ is first sampled from the prior $\pz$ and a value $\x$ is sampled from the conditional distribution $p_\theta(\x|\z)$.

A VAE can be used to simultaneously optimize the model's parameters and approximate the posterior, $p_\theta(\z|\x)$, via maximization of a lower bound on the marginal log-likelihood, 
\begin{equation}
\label{eq:VAEloss}
    \mathcal{L}(\theta,\phi)=\mathbb{E}_{\qzx}[\log \pxz)] - D_{KL}(\qzx)\Vert\pz),
\end{equation}
where the second term on the RHS is the Kullback-Leibler divergence~\cite{kullback1951information} from the true prior to an approximate posterior $\qzx$.
In \cref{eq:VAEloss}, the first term is known as the reconstruction error and the second term is known as the regularizer.
Consequently, $\qzx$ is known as the encoder, and $\pxz$ is known as the decoder.

\subsection{VAEs and the division of labour}
\label{sec:divlabour}
When designing a latent variable model for image data, the decoder can be made autoregressive, where the distribution of each pixel is conditioned on the value of previous pixels in row-major order, as well as on $\z$,
\begin{equation}
    \pxz=
    \prod^N_{i=1} \prod^M_{j=1}
    p_\theta(x_{i,j}|\z, x_{<(i,j)}).
    \label{eq:full-auto}
\end{equation}
We refer to $x_{<(i,j)}$ as the full AR \emph{receptive field}, and its shape is shown in \cref{fig:explainer}b.
This modification is intended to make the model more expressive.
However, the decoder is now powerful enough to model the entire data distribution locally,
to the extent that it is unclear which aspects of the data should be encoded in $\z$ and which should be modeled by the decoder.

In practice, when using a VAE, there seems to be a preference to  model as much content as possible with the decoder.
He~\etal~\cite{he2018lagging} argued this behaviour is caused by the approximate posterior lagging behind the true posterior in the early stages of training, causing the parameters to get stuck in a local optimum, where the decoder models the data without using the latent variables.

Alternatively, Chen~\etal~\cite{chenvariational} reasoned that with most practical VAEs, ignoring the latent variables achieves a tighter lower bound on the marginal loglikelihood.
By only using the latent variables to express what the decoder cannot model, the true posterior is brought closer to the prior and can be more closely matched by the relatively inflexible approximate posterior.
The authors then demonstrated how this behavior can be used to control the division of labor in a VAE.
Specifically, they designed an AR decoder that is capable of modeling information that they do not want captured in the latent variables, but is incapable of modeling the information that they do want captured in the latent variables.

In this paper, we design an AR receptive field that only captures the correlations common in scientific imaging noise.
This allows us to train a latent variable model of noisy image data where latent variables explain the signal content, and the decoder models only the noise generation process.
We then use the approximate posterior to sample latent variables, each representing one of the clean signals that could possibly underlie a given noisy image.

==> sections/intro-old.tex <==
\section{Introduction}
\label{sec:intro}

Microscopy has wide ranging applications in natural sciences.
As imaging technology is routinely pushed to its limits, microscopy images become affected by the presence of noise.
This poses a challenge in downstream analysis, making denoising an important preprocessing step.
Over the years, various denoising approaches have been devised~\cite{laine2021imaging}, from traditional filter-based methods~\cite{dabov2006image} to supervised deep learning-based methods~\cite{weigert2018content}.

Supervised deep learning-based methods excel with respect to the quality of their output, however, they require paired training data, typically consisting of pairs of noisy and clean images.
Unlike in applications with consumer images (photographs), such paired data is often unobtainable in microscopy~\cite{izadi2023image, song2021noise2void, xu2021deformed2self}.
Consequently, the applicability of supervised denoising methods in many areas of scientific imaging is limited.

Self- and unsupervised methods (\eg~\cite{batson2019noise2self,krull2019noise2void,prakash2020fully,prakashinterpretable,eom2023statistically}) have been proposed as a solution to the lack of high quality training data. 
They can be trained directly on the data that is to be denoised and have substantially improved the practical applicability of denoising in scientific imaging.
These methods separate the imaging noise from the underlying signal by making assumptions about the statistical nature of the noise.
Typically, they assume the noise is $(i)$ signal-independent (purely additive and occurs separately of the underlying signal)~\cite{salmon2022towards}, or $(ii)$ spatially uncorrelated (unstructured and occurs separately for each pixel)~\cite{krull2019noise2void, krull2020probabilistic, prakash2020fully, huang2021neighbor2neighbor, quan2020self2self}. 
We show examples of $(i)$ and $(ii)$ in \cref{fig:noisematrix}.

In practice, $(i)$ is often broken by the presence of Poisson shot noise~\cite{laine2021imaging}.
Moreover, many popular scientific cameras and imaging setups break $(ii)$ by producing row- or column-correlated noise.
For example, Scanning Transmission Electron Microscopy (STEM)~\cite{pennycook2011scanning} is prone to line artifacts caused by the slow reaction time of readout electronics~\cite{liao2006practical}, and Laser Scanning Confocal Microscopy (LSCM)~\cite{paddock2000principles} has been shown to produce artifacts in the scanning direction~\cite{herberich2012signal}.
Depending on their settings, Electron Multiplying Charge-Coupled Device (EMCCD)~\cite{denvir2003electron} cameras can produce horizontally correlated readout noise~\cite{broaddus2020removing}. 
The scientific Complementary Metal-Oxide-Semiconductor (sCMOS)~\cite{moomaw2013camera} cameras that are popular in optical microscopy~\cite{mandracchia2020fast} have separate amplifiers for each column of pixels, leading to correlated noise within each column~\cite{zhang2021characterizing}.
Additionally, the detectors used in infrared imaging systems, \eg microbolometers, also commonly use separate column amplifiers and suffer from similar noise structures~\cite{dupont2009fpn}. 
Examples of noisy images from these modalities along with plots of their spatial autocorrelation and signal-dependence can be found in \cref{fig:visResults}.
These types of noise cannot be removed with basic self- or unsupervised methods.
Recently, variants of these methods for spatially correlated noise have been proposed, but these are limited to locally correlated noise and can come at the expense of reduced reconstruction quality~\cite{broaddus2020removing,prakashinterpretable}.

In this paper, we present the first unsupervised deep learning-based denoiser capable of reliably removing signal-dependent noise that is correlated along rows or columns of pixels, as it commonly occurs in microscopy data.
The approach is illustrated in \cref{fig:explainer}.
Our method requires neither examples of noise-free images, which can be impossible to obtain (\eg~\cite{wang2020noise2atom}), nor pre-trained noise models~\cite{prakash2020fully, salmon2022towards, krull2020probabilistic} or hand-crafted priors~\cite{wang2020noise2atom, dabov2006image, gu2014weighted}.
Furthermore, we do not rely on blind-spot approaches~\cite{broaddus2020removing} or subsampling~\cite{huang2021neighbor2neighbor, lee2022ap} techniques that degrade image quality and therefore limit denoising performance.

The backbone of our approach is the Variational Autoencoder (VAE)~\cite{kingma2014auto}, which trains a latent variable model of the noisy image data $\x$ as $p_\theta(\x)\propto\pxz\pz$, where $\theta$ refers to the model parameters.
We guide our VAE to represent clean, noise-free images with latent variables $\z$ and to model the noise generation process with the decoder $\pxz$.

Our method for this is based on the representation learning technique proposed by Chen~\etal~\cite{chenvariational}, who revealed how a Variational Autoencoder (VAE)~\cite{kingma2014auto} prefers to avoid using latent variables $\z$ to describe structures that could instead be modeled locally by its decoder $\pxz$.
For an autoregressive (AR) decoder such as PixelCNN~\cite{van2016conditional, gulrajani2016pixelvae}, this includes any inter-pixel dependencies that lie within its receptive field.
Consequently, latent variables will only represent information that the decoder cannot model, \ie, dependencies that span beyond its receptive field.

We take advantage of this behavior by designing a decoder that is capable of modeling exactly what we want to be excluded from our latent variables -- the imaging noise -- while being incapable of modeling the remainder of the data.
Specifically, we use an AR decoder that can only model axis-aligned structures because its receptive field spans only a row or column of the image.
This trains our model to exclude row- or column-correlated noise from the latent variables, while encouraging it to include the statistics of the underlying signal.
We then propose a second network, termed \emph{signal decoder}, that is trained to map these latent variables back into the image space, thus producing denoised images.
Following Lehtinen~\etal~\cite{lehtinen2018noise2noise}, who showed that noisy images can be used as training targets for denoisers, we train the signal decoder alongside the VAE using the original noisy data as training targets.

\noindent To summarize, our main contributions are:
\begin{itemize}
    \item We present an unsupervised deep learning-based denoiser for signal-dependent noise that is correlated along rows or columns of pixels.
    \item By equipping a VAE with a 1-dimensional AR decoder, we guide it to represent clean images with latent variables and model noise content with the decoder.
    \item We introduce a novel architecture using a signal decoder that is trained in a second step to predict the signal from our latent variables.
    \item We apply our method to microscopy data recorded with various imaging modalities, as well as other datasets, achieving state-of-the-art denoising results compared to other unsupervised methods.
\end{itemize}

==> sections/related_work-old.tex <==
\section{Related work}
\subsection{Unsupervised denoising}
Existing unsupervised deep learning-based denoisers extend the latent variable model to include a known explicit noise model.
The joint distribution is then defined as
$p_\theta(\x,\s,\z)=p(\x|\s)p_\theta(\s|\z)p_\theta(\z)$,
where $p_\theta(\s|\z)$ is a deterministic distribution with support only at $g_\theta(\z)$ and $p(\x|\s)=p(\x|\s,\z)$.
The parameters of this model can be optimized by a VAE after a slight modification to the objective in \cref{eq:VAEloss}, changing the first term to $\mathbb{E}_{\qzx}[\log p(\mathbf{x}|\mathbf{s}=g_\theta(\mathbf{z}))]$.

In DivNoising~\cite{prakash2020fully}, the noise model follows \cref{eq:pixel-indep} and is learned from calibration data or co-learned during training. 
Later, HDN~\cite{prakashinterpretable} was proposed as an extension to DivNoising that used a VAE with a hierarchy of latent variables~\cite{sonderby2016ladder}.
It was found that short-range spatially correlated noise structures were modeled by only the bottom levels of the hierarchy, and they could be removed by preventing these latent variables from using information from the encoded input.
This technique is known as \hdn.

Next, Autonoise~\cite{salmon2022towards} was proposed to remove spatially correlated but signal-independent noise by replacing the pixel-independent noise model in HDN with a CNN-based AR decoder~\cite{van2016conditional}, $p(\x|\s)=\prod^N_{i=1} \prod^M_{j=1}p(x_{i,j}|\s, x_{<(i,j)})$.

Although this method can be used to remove noise of any spatial correlation, it cannot be applied to signal-dependent noise, making it inapplicable with most real-world data.
The reason for this is that the noise model must be pre-trained using suitable calibration data.
To learn only the structure of the noise, the calibration data required is samples of pure noise, which can be obtained by, \eg, imaging without light.
To also learn how the noise and signal are correlated, paired noisy and clean images with a range of signal content would be needed.
This is the same requirement as for supervised methods and rarely available.

\subsection{Self-supervised denoising}
Self-supervised deep learning-based denoisers use a noisy image as its own training target, but guide the network to learn a denoising function by corrupting the input in some way.
One technique~\cite{batson2019noise2self, krull2019noise2void, wang2022blind2unblind} introduces blind spots, forcing the network to predict the value of a pixel from surrounding pixels.
Another trains the network to predict a subset of randomly sampled pixels from another subset of randomly sampled pixels~\cite{huang2021neighbor2neighbor}.
For photon-counting data, Krull~\etal~\cite{krull2024image} proposed removing photons and training the network to predict them with a Poisson distribution.
These techniques exploit a property of spatially uncorrelated noise, which is that the noise in one pixel cannot be predicted from the noise in other pixels.

To address spatially correlated noise, the work Structured Noise2Void (SN2V)~\cite{broaddus2020removing} extended the blind-spot approach to also mask pixels containing noise that is correlated with the noise in the pixel being predicted.
Lee~\etal~\cite{lee2022ap} also extended the blind-spot approach, but by subsampling pixels to break up noise structures, making noise effectively spatially uncorrelated and ready for traditional blind-spot denoising.
N2V2~\cite{hock2022n2v2} constrained a blind-spot network's ability to reconstruct high-frequency information.


==> supp_figures.tex <==
\newcommand\tabSz{
    \begin{table}[]
    \centering
    \label{tab:Sz}
    \begin{tabular}{c:c|c}
    $f_\nu(\cdot)$ & $\overline{\x} : \x\sim p_\theta(\x|\cdot)$ & RMSE \\ \hline
    $\z^1$ & $\z^1$ & 2.43 \\
    $\z^2$ & $\z^2$ & 2.45 \\
    $\z^1$ & $\z^2$ & 23.28 \\
    $\z^2$ & $\z^1$ & 23.31 \\
    \end{tabular}
    \end{table}
}

\newcommand\figSz{
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{supp_figures/isszexz.pdf}
    \caption{Given a noisy image $\x$, we took two samples from the approximate posterior, $\z_1$ and $\z_2$.
    For each latent variable sample, we produced one estimate of the signal by passing it through the signal decoder $f_\nu$ and one by averaging 10,000 samples from the AR decoder, $\pxz$.}
    \label{fig:Sz}
\end{figure}
}

\newcommand\tabsampling{
\begin{table*}[h]
\centering
\caption{
Our denoiser randomly samples clean images for a given noisy image.
A consensus solution can be produced by averaging random samples.
The PSNR of the mean of increasing sample sizes is shown below.
}
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{l|ccc:ccc:cc}
\multicolumn{1}{l|}{} & \multicolumn{3}{c:}{EMCCD} & \multicolumn{3}{c:}{SCM} & \multicolumn{2}{c}{Simulated} \\
\multicolumn{1}{l|}{No. samples} & Conv. A & Conv. B & Mouse Actin & Mouse Nuclei* & Actin Conf. & Mito Conf.  & FFHQ Stripe  & FFHQ Checkerb. \\ \hline
 1 & 36.54 & 42.33 & 37.43 & 42.25 & 26.81 &  22.62 & 32.27 & 33.03\\
 10 & 37.39 & 43.90 & 39.03 & 42.91 & 27.37 & 23.39 & 35.24 & 35.85  \\
 100 & 37.49 & 44.10 & 39.23 & 42.98 & 27.42 & 27.50 & 35.66 & 36.27 \\
 1000 & 37.50 & 44.10 & 39.24 & 42.99 & 27.44 & 27.52 & 35.74 & 36.32\\
 \end{tabular}
 \end{adjustbox}
 \label{tab:sampling}
 \end{table*}
}

\newcommand\figConvA{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/conva-noisy.pdf}
    
    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/conva-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/conva-clean.pdf}
    \caption{\emph{Convallaria A}}
\end{figure*}
}

\newcommand\figConvB{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/convb-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/convb-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/convb-clean.pdf}
    \caption{\emph{Convallaria B}}
\end{figure*}
}

\newcommand\figMouseA{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/mouseactin-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/mouseactin-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/mouseactin-clean.pdf}
    \caption{\emph{Mouse Actin}}
\end{figure*}
}

\newcommand\figMouseN{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/mousen-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/mousen-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/mousen-clean.pdf}
    \caption{\emph{Mouse Nuclei}}
\end{figure*}
}

\newcommand\figActinConfocal{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/actinconfocal-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/actinconfocal-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/actinconfocal-clean.pdf}
    \caption{\emph{Actin Confocal}}
\end{figure*}
}

\newcommand\figMitoConfocal{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/mitoconfocal-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/mitoconfocal-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/mitoconfocal-clean.pdf}
    \caption{\emph{Mito Confocal}}
\end{figure*}
}

\newcommand\figEmbryo{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/embryo-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/embryo-denoised.pdf}
    \caption{\emph{Embryo}}
\end{figure*}
}

\newcommand\figStem{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/stem-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/stem-denoised.pdf}
    \caption{\emph{STEM}}
\end{figure*}
}

\newcommand\figInfrared{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/infrared-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/infrared-denoised.pdf}
    \caption{\emph{IR}}
\end{figure*}
}

\newcommand\figStripe{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/ffhqstripe-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/ffhqstripe-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/ffhqstripe-clean.pdf}
    \caption{\emph{FFHQ - Stripe}}
\end{figure*}
}

\newcommand\figCheckerboard{
\begin{figure*}[]
    \centering
    \includegraphics[width=0.8\linewidth]{supp_figures/noisy/ffhqcheckerboard-noisy.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/denoised/ffhqcheckerboard-denoised.pdf}

    \vspace{2mm}
    
    \includegraphics[width=0.8\linewidth]{supp_figures/clean/ffhqcheckerboard-clean.pdf}
    \caption{\emph{FFHQ - Checkerboard}}
\end{figure*}
}
